Multi-dimensional Preference Alignment by Conditioning Reward Itself

Reinforcement Learning from Human Feedback has emerged as a standard for aligning diffusion models. However, we identify a fundamental limitation in the standard DPO formulation because it relies on the Bradley-Terry model to aggregate diverse evaluation axes like aesthetic quality and semantic alignment into a single scalar reward. This aggregation creates a reward conflict where the model is forced to unlearn desirable features of a specific dimension if they appear in a globally non-preferred sample. To address this issue, we propose Multi Reward Conditional DPO (MCDPO). This method resolves reward conflicts by introducing a disentangled Bradley-Terry objective. MCDPO explicitly injects a preference outcome vector as a condition during training, which allows the model to learn the correct optimization direction for each reward axis independently within a single network. We further introduce dimensional reward dropout to ensure balanced optimization across dimensions. Extensive experiments on Stable Diffusion 1.5 and SDXL demonstrate that MCDPO achieves superior performance on benchmarks. Notably, our conditional framework enables dynamic and multiple-axis control at inference time using Classifier Free Guidance to amplify specific reward dimensions without additional training or external reward models.

==> main_before.tex <==
% hyperref with option pagebackref eases the reviewers' job, but should be disabled for the final version.
%
% If you comment hyperref and then uncomment it, you should delete
% main.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you
%  should be clear).

% TODO FINAL: Comment out the following line for the camera-ready version
%\usepackage[pagebackref,breaklinks,colorlinks,citecolor=eccvblue]{hyperref}
% TODO FINAL: Un-comment the following line for the camera-ready version
\usepackage{hyperref}

% Support for ORCID icon
\usepackage{orcidlink}
\usepackage{amsmath} % 수식 환경
\usepackage{amssymb}
\usepackage{kotex}
\usepackage{multirow}
\usepackage[normalem]{ulem}
\usepackage{wrapfig}
% \usepackage{svg}

\usepackage[table]{xcolor}

\useunder{\uline}{\ul}{}

\newcommand{\nj}[1]{{\color{red}#1}}

\input{cvpr/materials}

\begin{document}

% ---------------------------------------------------------------
% TODO REVIEW: Replace with your title
\title{Multi-dimensional Preference Alignment by Conditioning Reward Itself} 

% TODO REVIEW: If the paper title is too long for the running head, you can set
% an abbreviated paper title here. If not, comment out.
\titlerunning{Abbreviated paper title}

% TODO FINAL: Replace with your author list. 
% Include the authors' OCRID for the camera-ready version, if at all possible.
\author{First Author\inst{1}\orcidlink{0000-1111-2222-3333} \and
Second Author\inst{2,3}\orcidlink{1111-2222-3333-4444} \and
Third Author\inst{3}\orcidlink{2222--3333-4444-5555}}

% TODO FINAL: Replace with an abbreviated list of authors.
\authorrunning{F.~Author et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.

% TODO FINAL: Replace with your institution list.
\institute{Princeton University, Princeton NJ 08544, USA \and
Springer Heidelberg, Tiergartenstr.~17, 69121 Heidelberg, Germany
\email{lncs@springer.com}\\
\url{http://www.springer.com/gp/computer-science/lncs} \and
ABC Institute, Rupert-Karls-University Heidelberg, Heidelberg, Germany\\
\email{\{abc,lncs\}@uni-heidelberg.de}}

\maketitle


\begin{abstract}
Reinforcement Learning from Human Feedback has emerged as a standard for aligning diffusion models. 
However, we identify a fundamental limitation of the standard DPO formulation when optimizing multi-dimensional preferences: by relying on the Bradley-Terry model, it aggregates heterogeneous evaluation axes (e.g., aesthetic quality and semantic alignment) into a single scalar reward.
This aggregation creates a reward conflict where the model is forced to unlearn desirable features of a specific dimension if they appear in a globally non-preferred sample. To address this issue, we propose Multi Reward Conditional DPO (MCDPO) which resolves reward conflicts by introducing a disentangled Bradley-Terry objective. MCDPO explicitly injects a preference outcome vector as a condition during training, which allows the model to learn the correct optimization direction for each reward axis independently within a single network. We further introduce dimensional reward dropout to ensure balanced optimization across dimensions. Extensive experiments on Stable Diffusion 1.5 and SDXL demonstrate that MCDPO achieves superior performance on benchmarks even with 18\% and 3\% training data respectively.
Notably, our conditional framework enables dynamic and multiple-axis control at inference time using Classifier Free Guidance to amplify specific reward dimensions without additional training or external reward models.
  \keywords{DPO \and Diffusion \and Multi-preference}
\end{abstract}


\section{Introduction}
\label{sec:intro}

Reinforcement Learning from Human Feedback (RLHF)~\cite{ouyang2022rlhf}
% , a technique that aligns model outputs with human preferences,
has emerged as a key component in large-scale language model (LLM) training~\cite{liu2024deepseek,yang2025qwen3technicalreport,openai2025gptoss120bgptoss20bmodel}, 
and has recently been extended to generative image models~\cite{xu2023imagereward,lee2023aligning,black2023training}. Among these, Diffusion-DPO~\cite{wallace2024ddpo} applies Direct Preference Optimization (DPO)~\cite{rafailov2023dpo} to diffusion models using only binary win-lose labels via the Bradley-Terry (BT) model.

However, while a single image sample can possess various evaluation axes such as aesthetic quality, prompt fidelity, and safety, the BT model relies solely on a single win-lose label for the entire sample. This formulation makes it difficult to control or reflect specific, multi-dimensional preference axes during training.
This fundamental conflict arises from the standard BT model's formulation, which models global preference as a linear combination of multiple reward axes. 
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2mm}
\centering
\includegraphics[width=0.99\linewidth]{figure/mcdpo_concept3.pdf}
\vspace{-7mm}
\caption{DPO suffers from reward conflicts ($r^w-r^l < 0$) when global preference contradicts a specific dimension. MCDPO resolves this by disentangling axes to learn the correct direction for each dimension independently ($-(r^w-r^l) > 0$).}
\vspace{-7mm}
\label{fig:concept}
\end{wrapfigure}
Consequently, when presented with a sample pair that is a global \textit{win} but a local \textit{lose} on a specific dimension, % $j$, 
the model is forced to learn in the opposite direction of the intended preference for that dimension.
% Existing studies in the LLM field address this by: (1) dynamically combining model parameters based on reward weights~\cite{wang2024conditional}, (2) regularizing the gradients that align with the prior preference~\cite{lou2024spo}, or (3) in-context reward modeling via supervised fine-tuning (SFT)~\cite{yang2024rewards}.
% In the diffusion domain, a common strategy is to consider only the samples that are dominant across all axes as preferred~\cite{lee2025calibrated,gu2025paretohqd}.
% Nevertheless, these approaches fail to resolve the fundamental conflict within the DPO loss formulation. Consequently, they provide a limited learning signal and are sample-inefficient.
Prior works address this through parameter merging~\cite{wang2024conditional}, gradient regularization~\cite{lou2024spo}, SFT-based in-context reward modeling~\cite{yang2024rewards}, or filtering to conflict-free pairs~\cite{lee2025calibrated,gu2025paretohqd}, but none resolve the fundamental conflict within the DPO loss.

% In this work, we first propose a disentangled Bradley-Terry objective to resolve the issue. The core idea is to model preferences independently for each dimension by explicitly introducing a preference outcome vector that indicates the actual win, lose, or tie status for each axis. 
% This formulation ensures that every dimension is optimized in the correct direction by flipping the sign of the gradient term when a dimensional preference is inverted, thus resolving the ambiguity in conflicting pairs.

% The proposed method, Multi-reward Conditional Direct Preference Optimization (MCDPO), is the practical implementation of this objective.
% The key paradigm of MCDPO is to inject the preference outcome vector itself as a condition during the DPO loss calculation. 
% This approach transforms reward-conflict pairs into a powerful supervision signal, allowing the model to optimize each reward axis independently within a single network.

To resolve the issue, we propose a disentangled BT objective, which models preferences independently for each dimension by explicitly introducing a preference outcome vector that indicates the win, lose, or tie status for each axis. This formulation ensures every dimension is optimized in the correct direction, resolving the ambiguity in conflicting pairs. Our practical implementation, Multi-reward Conditional Direct Preference Optimization (MCDPO), injects this preference outcome vector itself as a condition during the DPO loss calculation, transforming problematic reward-conflict pairs into a powerful supervision signal for disentanglement within a single network (See \Cref{fig:concept}).
% This conditional approach transforms the problematic reward-conflict pairs into a powerful supervision signal for disentanglement, allowing the model to learn to optimize for each reward axis independently within a single network (See \Cref{fig:concept}).

By resolving the reward conflict, we experimentally demonstrate that MCDPO outperforms baselines and forms robust, efficient feature representations for each alignment axis.
Furthermore, the proposed conditional model provides a significant advantage at inference time. By leveraging the preference condition, the trained model can utilize Classifier-Free Guidance (CFG)~\cite{ho2022cfg} to measure and amplify the score function towards higher-reward outcomes, enabling dynamic, multi-axis control during generation.

In summary, the main contributions are as follows:
\vspace{-2mm}
\begin{itemize}
    \item We propose the disentangled BT objective and its practical implementation, Multi-reward Conditional DPO (MCDPO), to address the known reward conflict problem in BT-based DPO. Our method uses a preference outcome vector as a condition to disentangle reward axes.
    
    \item We experimentally show that MCDPO achieves superior performance and sample efficiency, learning robust representations for each alignment axis.
    
    \item We showcase MCDPO's conditional structure, which enables dynamic, multi-axis control during inference using Classifier-Free Guidance.
\end{itemize}

\section{Background}
\label{sec:background}

\subsection{Diffusion Models}

Diffusion models are a class of generative models that learn to generate data by reversing a gradual noising process.~\cite{ho2020denoising} The forward process progressively adds Gaussian noise to data $\mathbf{x}_0$ over $T$ timesteps:
\begin{equation}
q(\mathbf{x}_t|\mathbf{x}_{t-1}) = \mathcal{N}(\mathbf{x}_t; \sqrt{1-\beta_t}\mathbf{x}_{t-1}, \beta_t\mathbf{I}),
\end{equation}
where $\beta_t$ is a variance schedule. The reverse process learns to denoise by training a network $\epsilon_\theta$ to predict the noise at each timestep. The training objective is:
\begin{equation}
\mathcal{L} = \mathbb{E}_{t, \mathbf{x}_0, \epsilon}\left[\|\epsilon - \epsilon_\theta(\mathbf{x}_t, t, c)\|^2\right],
\end{equation}
where $c$ represents conditioning information (e.g., text prompt), and $\epsilon \sim \mathcal{N}(0, \mathbf{I})$ is the added noise to $\mathbf{x}_0$.

At inference, sampling starts from pure noise $\mathbf{x}_T \sim \mathcal{N}(0, \mathbf{I})$ and iteratively denoises to generate $\mathbf{x}_0$. The learned score function $\nabla_{\mathbf{x}} \log p_\theta(\mathbf{x}_t|c)$ guides this reverse process~\cite{song2020score}. 
Classifier-Free Guidance (CFG)~\cite{ho2022cfg} strengthens conditioning by modifying the score function:
\begin{small}
\begin{equation}
% \nabla_{\mathbf{x}} \log \tilde{p}_\theta(\mathbf{x}_t|c) = 
\nabla_{\mathbf{x}} \log p_\theta(\mathbf{x}_t) + \lambda_{\text{cfg}} \left(\nabla_{\mathbf{x}} \log p_\theta(\mathbf{x}_t|c) - \nabla_{\mathbf{x}} \log p_\theta(\mathbf{x}_t)\right),
\end{equation}
\end{small}
%\normalsize
where $\lambda_{\text{cfg}}$ controls guidance strength. By amplifying the score difference, CFG enhances adherence to the conditioning signal $c$.

\subsection{DPO in Diffusion Models}
% % 
% \begin{equation}
%     p_{BT}(x^w>x^l|c) = \sigma(r(x^w, c)-r(x^l, c))
%     \label{eq:BT}
% \end{equation}

% \begin{equation}
%     r(x,c) = \beta log(\frac{p_\theta(x|c)}{p_{ref}(x|c)}) + \beta logZ(c)
%     \label{eq:reward}
% \end{equation}

% \footnotesize
% \begin{equation}
%     L = -\mathbb{E} \ log\sigma \left( \beta log\frac{p_\theta(x_t^w|x_{t+1}^w,c)}{p_{ref}(x_t^w|x_{t+1}^w,c)}-\beta log\frac{p_\theta(x_t^l|x_{t+1}^l,c)}{p_{ref}(x_t^l|x_{t+1}^l,c)} \right)
%     \label{eq:dpo_loss}
% \end{equation}
% \normalsize

Direct Preference Optimization (DPO)~\cite{rafailov2023dpo} offers a simplified approach to align generative models with human preferences by directly optimizing policy models without requiring explicit reward models. DPO leverages the Bradley-Terry (BT) model~\cite{bradley1952rank} to model preference probabilities from pairwise comparisons. Given a pair of samples $\mathbf{x}^w$ (preferred) and $\mathbf{x}^l$ (less preferred) conditioned on prompt $c$, the BT model defines:
\begin{equation}
p_{\text{BT}}(\mathbf{x}^w > \mathbf{x}^l | c) = \sigma(r(\mathbf{x}^w, c) - r(\mathbf{x}^l, c)),
\end{equation}
where $\sigma(\cdot)$ is the sigmoid function and $r(\mathbf{x}, c)$ is a reward function.

A key insight of DPO is that the reward can be expressed analytically in terms of the learned policy $p_\theta$ and a reference policy $p_{\text{ref}}$:
\begin{equation}
r(\mathbf{x}, c) = \beta \log \left(\frac{p_\theta(\mathbf{x}|c)}{p_{\text{ref}}(\mathbf{x}|c)}\right) + \beta \log Z(c),
\end{equation}
where $\beta$ is a KL regularization parameter and $Z(c)$ is the partition function. This formulation allows DPO to optimize preferences directly through the policy without training a separate reward model.

For diffusion models~\cite{wallace2024ddpo}, the DPO objective operates at the denoising transition level. Given a preference (win-lose) pair $(\mathbf{x}^w, \mathbf{x}^l)$, the loss function is:
\begin{footnotesize}
\begin{equation}
\begin{split}
\mathcal{L}_{\text{DPO}} =& -\mathbb{E} \log \sigma \left( \beta \log \frac{p_\theta(\mathbf{x}^w_t|\mathbf{x}^w_{t+1}, c)}{p_{\text{ref}}(\mathbf{x}^w_t|\mathbf{x}^w_{t+1}, c)} - \beta \log \frac{p_\theta(\mathbf{x}^l_t|\mathbf{x}^l_{t+1}, c)}{p_{\text{ref}}(\mathbf{x}^l_t|\mathbf{x}^l_{t+1}, c)} \right) \\
=& -\mathbb{E} \log \sigma (-\beta T \omega_t\ (||\epsilon^w - \epsilon_\theta(\mathbf{x}_t^w,t)||^2 - ||\epsilon^w - \epsilon_\text{ref}(\mathbf{x}_t^w,t)||^2 \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ - (||\epsilon^l - \epsilon_\theta(\mathbf{x}_t^l,t)||^2 - ||\epsilon^l - \epsilon_\text{ref}(\mathbf{x}_t^l,t)||^2)
),
\end{split}
\end{equation}
\end{footnotesize}
where the expectation is over timesteps $t$ and noisy samples from the diffusion forward process. This formulation trains the diffusion model to increase the likelihood of preferred samples while decreasing that of less preferred ones, relative to the reference policy.

% \subsection{Multi-dimensional Reward}

% 일반적으로 image나 text와 같은 generated sample을 평가하는 데에는 여러가지 aspect가 동시에 고려된다. (e.g. aesthetic, text-alignment, helpfulness, harmlessness)
% 하지만 하나의 scalar 값으로 reward를 modeling하는 bradley-terry의 특성으로 인해, global reward가 여러 reward의 linear combination으로 정의된다고 생각할 수 있다.

% % equation으로 할지 inline으로 할지 확인 필요
% \begin{equation}
%     r(x,c) = \sum_i w_ir_i(x,c)
%     \label{eq:multi-reward}
% \end{equation}

% $x^w$ $x^l$은 image pair에서 global reward에서 win, lose하는 sample.
% 하지만 이는 practically 많은 경우 reward conflict를 야기한다. 예를 들어, $r_1$이 text-alignment, $r_2$가 aesthetic score에 대한 reward라고 하고, 두 aspect가 align되지 않았을 때 $r_1(x^w) > r_1(x^l), r_2(x^w) < r_2(x^l)$, eq~\ref{eq:dpo_loss}를 통해서 학습하면, $r_2$, aesthetic score는 오히려 더 나빠지는 쪽으로 학습되게 된다.~\ref{}

% 이를 해결하기위해 existing work 들은 significantly 많은 sampling을 통해 dominate한 pair를 만들거나 pareto-front를 찾아서 학습한다.
% 하지만 이는 pickapicv2같은 dataset를 활용한 offline dpo를 통해 학습할 수 없다

In practice, generated samples are evaluated along multiple distinct axes, such as aesthetic quality, semantic alignment, and safety. However, the standard BT model aggregates these into a single scalar reward by a linear combination of different dimensions:
%, effectively modeling the global reward as a linear combination:
\begin{equation}
r(\mathbf{x}, c) = \sum_{i=1}^D w_i r_i(\mathbf{x}, c),
\end{equation}
where $r_i$ represents the reward for dimension $i$ and $w_i$ its weight. This leads to a fundamental reward conflict: when $x^w$ is preferred globally but performs worse than $x^l$ on a specific dimension $j$, the DPO loss may inadvertently degrade that dimension as shown in \Cref{fig:concept} (Left). 
% While, 이전 연구들이 이러한 방식으로 reward conflicts를 해결하려 하지만, 펀더멘털하게 해소하지 못한다 블라블라.

Existing studies attempt to address or bypass this issue. In the LLM field, prominent approaches include: (1) dynamically combining expert model parameters based on user-specified reward weights~\cite{wang2024conditional}, (2) %train the model sequentially by applying regularization to align gradients with prior preferences~\cite{lou2024spo}, or (3) circumventing the DPO conflict entirely by using Supervised Fine-Tuning (SFT) leverages reward scores within the prompt~\cite{yang2024rewards}.
training sequentially with regularization that encourages gradient alignment with previously learned preferences~\cite{lou2024spo}, and (3) avoiding DPO conflicts by using supervised fine-tuning (SFT) that incorporates reward scores directly in the prompt~\cite{yang2024rewards}.
In the diffusion domain, a common strategy to avoid this conflict is to generate images until the samples that are dominant across all axes as preferred~\cite{lee2025calibrated,gu2025paretohqd}.
Nevertheless, these approaches fail to resolve the fundamental conflict within the DPO loss formulation itself. By either training only on non-conflicting pairs (which is sample-inefficient) or using alternative objectives (like SFT or regularization), they rely on a limited learning signal rather than directly solving the ambiguity in DPO.
In this work, we aim to analyze the problem and resolve the limitations.



\section{Method}
\label{sec:method}
% in this section, 우리 알고리즘을 소개한다. 우리는 기존의 reward conflict 문제를 reward를 disentangle을 통해 모든 dimension에서 preferrable하게 학습할 수 있는 $p^\perp_{BT}$를 정의하고, $p^\perp_{BT}$를 dpo로 학습하기 위해서 reward 자체를 input condition으로 활용하는 Multi-reward Conditional DPO (MCDPO)를 제안한다. 이때 특정 reward dimension이 $p^\perp_{BT}$를 dominate할 수 있는 문제가 있을 수 있음을 보이며, 이를 해결할 수 있는 dimensional reward drop방법을 제안한다. 그리고 mcdpo가 cfg를 통해, test-time에 reward를 높이는 score function을 modeling할 수 있음을 보인다.
% 2.3 빼버리고 diffusion, dpo만 얘기하고 더 필요한 bg있으면 넣는게 좋을듯
% 2.3은 3장으로 가져오는게 나을거같음 흐름은:
% [A] method intro 넣을거면 
% 이 섹션에서 우리는 한 샘플에 여러 리워드 축이 정의된 상황 (multi-dimensional reward)에서 기존 BT modeling을 활용하는 DPO의 objective function이 reward conflict 문제로부터 자유롭지 못함을 먼저 보인다. 이후 이를 극복하기 위해 reward conditioning 기반의 접근인 Multi-reward Conditional DPO (MCDPO)를 derive 한다. 우리는 제안 방법의 구현이 비교적 간단함에도 불구하고 이론적 배경을 토대로 reward dimension을 disentangle하여 더 나은 learning signal을 제공할 뿐만 아니라 sampling time에서 또한 score guiding을 통해 preference를 극대화하는 방법을 소개한다. ... 

% [B] method intro 없이 바로 시작 / subsection 제목은 문제 강조를 위해 약간 변경 필요할듯
% \subsection{Analysis on Multi-dimensional DPO} 
% 2.3 내용을 여기로 옮기고 ( Multi-dimensional Reward conflict 난다는거)
% 3.1의 Disentangled Bradley-Terry Objective 도 여기로 오고

% subsection 제목은 MCDPO 보다는 어떤 문제를 conditioning으로 해결할거다가 되면 좋을듯
% 3.4의 내용을 좀 간소화 시켜서 여기 마지막에 붙이거나 걍 실험섹션으로 넘겨도될듯
% \subsection{... by Conditioning}
% 우리는 앞서 분석한 문제의 완화를 위한 효과적인 해법으로 conditioning을 통해 $p^{\perp}_{BT}$ 를 근사하는 MCDPO를 제안한다:
% eq10

% 이는 각 샘플에 대한 각 리워드 점수 자체를 condition으로 제공함으로써 모델이 각 dimension에 대한 disentangled repr를 학습하도록 유도한다.
% 이는 모델로 하여금 condition으로 제공된 $\gamma$를 기반으로 인풋에 대하여 각 리워드 축에 대해 explicitly 파악할 수 있게된다. 
% (여긴 복붙)
% This transforms conflict pairs into supervision for disentanglement: when $\gamma = [\text{aesthetic: win, semantic: lose}]$, the model must learn that aesthetics favors $x^w$ while semantics favors $x^l$—possible only if these dimensions are represented independently. When such conflict pairs are sufficiently represented, the model learns to disentangle each reward dimension, effectively training $D$ implicit reward models $r_i(x, c)$ within a single network.
% 구체적으로 우리는 다음과 같이 symmetry of preference를 활용하는 방식으로 다음의 loss function을 정의한다:
% \begin{equation}
% \footnotesize
% \begin{split}
% \footnotesize
%     L_{MC} = -\mathbb{E}\ log\sigma \Biggl[ \beta\Biggl( &log\frac{p(x^w|c,\gamma(x^w,x^l))}{p_{ref}(x^w|c)} - log\frac{p(x^l|c,\gamma(x^w,x^l))}{p_{ref}(x^l|c)} \Biggl)\\
%     + \beta\Biggl(& log\frac{p(x^l|c,\gamma(x^l,x^w))}{p_{ref}(x^l|c)} - log\frac{p(x^w|c,\gamma(x^l,x^w))}{p_{ref}(x^w|c)} \Biggl)\Biggl]
% \end{split}
% \end{equation}
% 우리는 이러한 방식으로 하나의 샘플에 대한 global reward를 정의하기 어려운 d1= win, d2=lose case와 같은 sample에서 또한 적절한 learning signal을 제공할 수 있게 된다. %% data efficiency 얘기는 실험 + intro에서 간략히 언급하는게 나을듯

% 기본 제목은 방법 그 자체(리워드드랍아웃)인데 그거보단 subsection title이 어떤 learnable query로 교체 하는 것 보다 tie(0)으로 바꾸는게 낫다는게 강조될 수 있으면 좋을듯
% \subsection{Gradient Domination and Reward Neutralization}
% 지금 적힌 3.2도 ㄱㅊ은거같은데:
% multi-dimensional reward 학습을 eq11처럼 만들게 되면 multi-objectives를 갖게 되고 (or 일종의 multi-task learning이 된다-- 이건 reference있으면 가능할듯), 하나의 reward에 대한 학습이 용이한 경우 다른 축들에 대한 학습이 발생하기 전에 local optima로 수렴하는 문제가 발생할 수 있다.
% 구체적으로 제안된 obj의 gradient는 다음과 같다.
% \begin{equation}
% \begin{split}
% \footnotesize
%     &\nabla_\theta L_M = (\sigma (z)-1)\nabla_\theta z, \\
%     &\nabla_\theta z = \sum_i\beta w_i (\nabla_\theta log p_\theta(x^w|c,\hat\gamma_i) - \nabla_\theta log p_\theta(x^l|c,\hat\gamma_i))
% \end{split}
% \end{equation}
% where z, ... = ㅇㅇ, respectively.
% 이때 The problem arises from two sources: (1) if any single dimension becomes 
% highly confident, $\sigma(z) \to 1$ shrinks the global gradient to zero, 
% stalling all dimensions, and (2) within $\nabla_\theta z$, if the model 
% becomes highly discriminative for dimension $i$, which causes a large gradient norm for that dimension, 
% it can dominate the sum and overwhelm gradients from other dimensions.
% 우리는 이러한 문제를 완화하고자 각 reward dimension에 대해 독립적으로 reward을 0으로 set하는 방식으로 dropout을 수행한다. This prevents any dimension from consistently dominating, ensuring balanced optimization across all axes.
% 3.3은 원래대로
% 3.4의 내용을 좀 간소화 시켜서 3.2 마지막에 붙이거나 걍 실험섹션으로 넘겨도될듯

% In this section, we describe a framework to address the reward conflict inherent in multi-dimensional DPO. We begin by theoretically analyzing this conflict and then introduce a disentangled Bradley-Terry objective that fundamentally resolves it in \Cref{subsec:reward_conflict}. 
% Following this analysis, we introduce Multi-reward Conditional DPO (MCDPO) in \Cref{subsec:mcdpo} that leverages reward conditioning to approximate this theoretical objective using a single network. 
% To ensure balanced optimization, in \Cref{subsec:reward_drop}, we identify the potential issue of gradient domination and propose reward dropout as a robust solution. Finally, in \Cref{subsec:testtime}, we demonstrate how our conditional framework uniquely enables dynamic, multi-axis test-time reward optimization.
We first analyze the reward conflict and propose a disentangled BT objective (\Cref{subsec:reward_conflict}), then introduce MCDPO as its practical single-network implementation (\Cref{subsec:mcdpo}), address gradient domination via reward dropout (\Cref{subsec:reward_drop}), and show how our conditional framework enables test-time reward control (\Cref{subsec:testtime}).


\subsection{Multi-reward Disentanglement}
\label{subsec:reward_conflict}
% Generated samples are often evaluated along multiple, distinct axes, such as aesthetic quality, prompt fidelity, or safety. 
% Standard Direct Preference Optimization (DPO), which leverages the Bradley-Terry (BT) model, struggles in this multi-dimensional setting. 
As discussed in \Cref{sec:background}, the standard BT model collapses multi-dimensional
preferences into a single scalar preference:
\begin{equation}
    p_{BT}(\mathbf{x}^w>\mathbf{x}^l|c)
    =
    \sigma\!\left[\sum_i w_i\big(r_i(\mathbf{x}^w,c)-r_i(\mathbf{x}^l,c)\big)\right].
\end{equation}
This formulation leads to a reward conflict when a sample $\mathbf{x}^w$ is globally preferred over $\mathbf{x}^l$, but is worse than $x^l$ on a particular dimension $j$, (i.e.,
$r_j(\mathbf{x}^w,c) < r_j(\mathbf{x}^l,c)$).
Because the standard DPO loss optimizes only for the global win, it inadvertently compels the model to learn in the opposite direction for dimension $j$, actively degrading that specific quality.
To resolve this, we first introduce a disentangled Bradley-Terry objective. The core idea is to model the preference for each dimension. We explicitly introduce a pairwise preference outcome vector $\gamma(\mathbf{x},\mathbf{y}) \in \{-1,0,1\}^D$, where each entry indicates whether $\mathbf{x}$ wins, loses, or ties against $\mathbf{y}$ on reward axis $i$, \ie, $\gamma_i(x,y) = \text{sign}(r_i(x) - r_i(y))$.
% \small
% \begin{equation}
%   %   \gamma_i(x,y) = \begin{cases}
%   %       1 & \text{if } r_i(x) > r_i(y) \\
%   % 0 & \text{if } r_i(x) = r_i(y) \\
%   % -1 & \text{if } r_i(x) < r_i(y) .
%   %   \end{cases}

% \end{equation}
% \normalsize
Using $\gamma$, we define the disentangled Bradley-Terry $p^\perp_{BT}$ target:
\footnotesize
\begin{equation}
\begin{split}
    p^\perp_{BT}(\mathbf{x}^w>\mathbf{x}^l \mid c,\gamma(\mathbf{x}^w,\mathbf{x}^l))
    =
    \sigma\!\left[
    \sum_i w_i \gamma_i(\mathbf{x}^w,\mathbf{x}^l)
    \big(r_i(\mathbf{x}^w,c)-r_i(\mathbf{x}^l,c)\big)
    \right].
\end{split}
\label{eq:disentangle_bt}
\end{equation}
\normalsize

Eq.~\eqref{eq:disentangle_bt} specifies the desired preference probability once the per-dimension outcomes are known.
This formulation ensures each dimension is optimized in the correct direction. In particular, if the $j$-th dimensional preference is inverted (e.g., $\mathbf{x}^l$ wins on aesthetics), $\gamma_j$ becomes negative, which flips the sign for that dimension's contribution. By doing so, we can resolve the sign ambiguity in conflicting pairs and provide correct supervision across all dimensions.

\subsection{Multi-reward Conditional DPO}
\label{subsec:mcdpo}
Because standard DPO is structurally limited to modeling a single reward axis, modeling multiple axes would require training multiple separate implicit reward diffusion models.
\begin{equation}
    r_i(\mathbf{x},c) = \beta \log\left(\frac{p_i(\mathbf{x}|c)}{p_\text{ref}(\mathbf{x}|c)}\right) + \beta \log Z(c)
\end{equation}
this approach would require optimizing a loss:
\footnotesize
\begin{equation}
    L_M = -\mathbb{E}\ \log\sigma\left[\beta \sum_iw_i\gamma_i \left( \log\frac{p_i(\mathbf{x}^w|c)}{p_{\text{ref}}(\mathbf{x}^w|c)} - \log\frac{p_i(\mathbf{x}^l|c)}{p_{\text{ref}}(\mathbf{x}^l|c)}\right)\right],
    \label{eq:lm}
\end{equation}
\normalsize 
which has two major drawbacks. First, it does not fundamentally resolve conflicts, as each model is still trained on pairs where its dimension may conflict with others.
Second, it requires training $D$ separate models which is computationally prohibitive.
%While the first issue can be addressed by introducing the per-dimension preference indicator $i$ from our disentangled BT objective~\eqref{eq:disentangle_bt}, and the separate models can be compressed into a single network conditioned on dimension indicator $i$:
The first issue can be addressed by incorporating the per-dimension preference indicator $i$ from our disentangled BT objective \eqref{eq:disentangle_bt}, and the separate models can be further consolidated into a single network conditioned on $i$:
\footnotesize
\begin{equation}
    L_M' = -\mathbb{E}\ \log\sigma\left[\beta \sum_iw_i\gamma_i \left( \log\frac{p(\mathbf{x}^w|c,i)}{p_{\text{ref}}(\mathbf{x}^w|c)} - \log\frac{p(\mathbf{x}^l|c,i)}{p_{\text{ref}}(\mathbf{x}^l|c)}\right)\right].
    \label{eq:lm_prime}
\end{equation}
\normalsize 
%this formulation resolves the reward conflict, as conditioning on $i$ ensures each dimension is optimized in its correct direction. 
This formulation effectively resolves reward conflicts, as conditioning the model on $i$ ensures that each specific quality dimension is optimized in its intended direction.
However, it remains computationally prohibitive. The summation inside the sigmoid requires evaluating the log-likelihood ratio independently for each dimension $i$, necessitating $D$ separate forward-backward passes per training step.

% To resolve this, we propose Multi-reward Conditional DPO (MCDPO), an efficient solution that effectively models $p_{BT}^\perp$ using a single conditional diffusion model. The key insight is to inject the preference outcome vector $\gamma$ itself as a condition during training.

% \vspace{-2mm}
% \footnotesize
% \begin{equation}
%     \sigma\left(\beta \log \frac{p(\mathbf{x}^w|c,\gamma(\mathbf{x}^w,\mathbf{x}^l))}{p_{\text{ref}}(\mathbf{x}^w|c)} - \beta \log \frac{p(\mathbf{x}^l|c,\gamma(\mathbf{x}^w,\mathbf{x}^l))}{p_{\text{ref}}(\mathbf{x}^l|c)}\right) \approx p_{BT}^\perp.
% \end{equation}
% \normalsize

%%%%%%%%%%%%%%%%%%
To resolve this, we propose Multi-reward Conditional DPO (MCDPO), an efficient solution that models $p_{BT}^\perp$~\eqref{eq:disentangle_bt} using a single conditional diffusion model.
Following DPO, we interpret the policy/reference log-ratio as an implicit reward, but make it conditional on the pairwise outcome vector $\gamma$:
% \begin{equation}
% \footnotesize
%     \sigma\left(\beta log \frac{p(x^w|c,\gamma(x^w,x^l))}{p_{ref}(x^w|c)} - \beta log \frac{p(x^l|c,\gamma(x^w,x^l))}{p_{ref}(x^l|c)}\right) \approx p_{BT}^\perp
% \end{equation}
\begin{equation}
    r_\theta(\mathbf{x},c,\gamma)
    =
    \beta \log \frac{p_\theta(\mathbf{x}\mid c,\gamma)}{p_{\mathrm{ref}}(\mathbf{x}\mid c)} + \beta \log Z(c,\gamma).
\end{equation}
This induces a conditional Bradley-Terry probability
\begin{equation}
\begin{split}
    \hat p_\theta^\perp&(\mathbf{x}^w>\mathbf{x}^l \mid c,\gamma)
    =
    \sigma\!\left(
    r_\theta(\mathbf{x}^w,c,\gamma)-r_\theta(\mathbf{x}^l,c,\gamma)
    \right)
    \\&=
    \sigma\!\left(
    \beta \log \frac{p_\theta(\mathbf{x}^w\mid c,\gamma)}{p_{\mathrm{ref}}(\mathbf{x}^w\mid c)}
    -
    \beta \log \frac{p_\theta(\mathbf{x}^l\mid c,\gamma)}{p_{\mathrm{ref}}(\mathbf{x}^l\mid c)}
    \right).        
    \end{split}
    \label{eq:conditional_bt}
\end{equation}
% where the goal is to train a single conditional policy $p_\theta(\mathbf{x}\mid c,\gamma)$ such that its induced preference probability $\hat p_\theta^\perp$ approximates the disentangled target $p^\perp_{BT}$ in Eq.~\eqref{eq:disentangle_bt}.

% Under sufficient model capacity, the conditional implicit reward $r_\theta(\mathbf{x}, c, \gamma)$ 
% can represent the disentangled reward structure. Specifically, since $\gamma$ takes values 
% in a finite discrete set $\{-1,0,1\}^D$, the conditional policy $p_\theta(\mathbf{x}|c,\gamma)$ 
% can, in principle, learn a distinct implicit reward function for each value of $\gamma$. 
% At the optimum $\theta^*$, the induced reward satisfies:
% \begin{equation}
% r_{\theta^*}(\mathbf{x}, c, \gamma) = \sum_i w_i \gamma_i\, r_i(\mathbf{x}, c) + g(c, \gamma),
% \label{eq:reward_decomp}
% \end{equation}
% where $g(c, \gamma)$ is independent of $\mathbf{x}$ and thus cancels in the pairwise difference 
% $r_{\theta^*}(\mathbf{x}^w, c, \gamma) - r_{\theta^*}(\mathbf{x}^l, c, \gamma)$. 
% Substituting this into Eq.~\eqref{eq:conditional_bt} recovers the disentangled target 
% $p^\perp_{BT}$ in Eq.~\eqref{eq:disentangle_bt}, establishing $\hat{p}^\perp_{\theta^*} = p^\perp_{BT}$.


Under sufficient model capacity and an expressive conditioning mechanism,
the conditional policy $p_\theta(\mathbf{x}|c,\gamma)$ can, in principle, learn
a distinct implicit reward function for each value of $\gamma \in \{-1,0,1\}^D$.
% We now show that the optimum takes a specific decomposed form.

Let $r_{\text{eff}}(\mathbf{x}, c, \gamma) \triangleq \sum_i w_i \gamma_i\, r_i(\mathbf{x}, c)$ be the effective reward under condition $\gamma$. 
By construction, the effective reward difference
satisfies:
\footnotesize
\begin{equation}
r_{\text{eff}}(\mathbf{x}^w, c, \gamma) - r_{\text{eff}}(\mathbf{x}^l, c, \gamma)
%= \sum_i w_i \gamma_i (r_i(\mathbf{x}^w, c) - r_i(\mathbf{x}^l, c))
= \sum_i w_i |r_i(\mathbf{x}^w, c) - r_i(\mathbf{x}^l, c)| \geq 0,
\label{eq:consistency}
\end{equation}
\normalsize
which guarantees that the training label ($\mathbf{x}^w$ preferred) is consistent with the effective reward $r_{\text{eff}}(\mathbf{x}, c, \gamma)$ %$ \triangleq \sum_i w_i \gamma_i\, r_i(\mathbf{x}, c)$
under the Bradley-Terry model for every $\gamma$. Since each fixed $\gamma$ reduces $L_{MC}$ (Eq.~\eqref{eq:lmc}) to a standard DPO objective with ground-truth reward $r_{\text{eff}}$, the DPO optimality result~\cite{rafailov2023dpo} directly implies that at the optimum $\theta^*$, the  induced reward satisfies:
\begin{equation}
r_{\theta^*}(\mathbf{x}, c, \gamma) = \sum_i w_i \gamma_i\, r_i(\mathbf{x}, c) + g(c, \gamma),
\label{eq:reward_decomp}
\end{equation}
where $g(c, \gamma)$ is independent of $\mathbf{x}$ and thus cancels in the pairwise difference
$r_{\theta^*}(\mathbf{x}^w, c, \gamma) - r_{\theta^*}(\mathbf{x}^l, c, \gamma)$.
Substituting this into Eq.~\eqref{eq:conditional_bt} recovers the disentangled target
$p^\perp_{BT}$ in Eq.~\eqref{eq:disentangle_bt}, establishing
$\hat{p}^\perp_{\theta^*} = p^\perp_{BT}$. 

Intuitively, the training dynamics naturally drive the model toward this decomposition. Consider a conflicting pair where $\gamma=[\text{aesthetic: $+1$},\ \text{semantic: $-1$}]$. The loss requires the model to increase the likelihood of $\mathbf{x}^w$ along the aesthetic axis while \emph{decreasing} it along the semantic. The same pair also appears with the flipped condition $\gamma=[\text{aesthetic: $-1$},\ \text{semantic: $+1$}]$ via our final symmetric loss Eq.~\eqref{eq:lmc}, which imposes the opposite constraint. To satisfy both simultaneously, the model must learn to modulate its implicit reward for each dimension independently as a function of $\gamma$, which is precisely the structure captured by Eq.~\eqref{eq:reward_decomp}:
While Eq.~\eqref{eq:reward_decomp} may not hold exactly in practice due to the finite capacity of the conditioning mechanism,~\Cref{tab:implicit} empirically validates that our architecture approximates this decomposition well. The single MCDPO model achieves implicit reward accuracy comparable to specialist models trained on individual dimensions.
% We empirically verify this in~\Cref{tab:implicit} shows that our single conditional model achieves implicit reward accuracy comparable to specialist models trained on individual dimensions.
% \vspace{-4mm}
\footnotesize
\begin{equation}
\begin{split}
    L_{MC} = -\mathbb{E}\ \Biggl[ \log\sigma \Biggl( &\beta \log\frac{p(\mathbf{x}^w|c,\gamma^{wl})}{p_{\text{ref}}(\mathbf{x}^w|c)} - \beta \log\frac{p(\mathbf{x}^l|c,\gamma^{wl})}{p_{\text{ref}}(\mathbf{x}^l|c)} \Biggl)\\
    + \log\sigma\Biggl(&\beta \log\frac{p(\mathbf{x}^l|c,\gamma^{lw})}{p_{\text{ref}}(\mathbf{x}^l|c)} - \beta \log\frac{p(\mathbf{x}^w|c,\gamma^{lw})}{p_{\text{ref}}(\mathbf{x}^w|c)} \Biggl)\Biggl],
\end{split}
\label{eq:lmc}
\end{equation}
\normalsize
where $\gamma^{wl}$ and $\gamma^{lw}$ denote $\gamma(x^w,x^l)$ and $\gamma(x^l,x^w)$, respectively. To feed $\gamma$ into the model, we devise a reward conditioning module described in \Cref{subsec:contextawaremodule}.

% The key insight is to reframe the objective from an explicit sign-flip (\Cref{eq:lm}) to a learned function approximation task. We leverage the core DPO principle that the policy is an implicit reward model, but define a conditional implicit reward: $r_\theta(\mathbf{x},c,\gamma) = \beta \log(p(\mathbf{x}|c,\gamma)/p_\text{ref}(\mathbf{x}|c))$. Our final loss, $L_{MC}$ (\Cref{eq:lmc}), trains this single $r_\theta(\mathbf{x},c,\gamma)$ to emulate the behavior of the entire theoretical, disentangled ensemble from~\Cref{eq:lm}.
%%%%%%%%%%%%%%%%%%


% By conditioning on $\gamma$, conflicting pairs become informative supervision rather than ambiguous preference labels. For example, when the model is given a pair with $\gamma = [\text{aesthetic: win, semantic: lose}]$, it should learn to recognize that $x^w$ is aesthetically superior, while $x^l$ has better semantic alignment. 

% Conditioning on $\gamma$ makes conflicting pairs informative rather than ambiguous by explicitly specifying the preferred direction on every reward axis.
% For example, if $\gamma=[\text{aesthetic: win},\ \text{semantic: lose}]$, the model is told that $\mathbf{x}^w$ should be preferred on the aesthetic axis while $\mathbf{x}^l$ should be preferred on the semantic axis.
% Thus, MCDPO turns the disentangled multi-model objective in Eq.~\eqref{eq:lm} into a single conditional function approximation problem.

% It is only possible if the model learns to represent these preference axes independently. 
% When trained on sufficient conflict pairs, the model learns to disentangle each reward dimension, effectively training $D$ implicit reward models within a single model. 


% To maximize data efficiency, our final loss function, $L_{MC}$, exploits the symmetry of preferences by training on both pair orientations as follows:


% a simple parallel cross-attention mechanism is insufficient, as dimensions like semantic alignment require comparing the text prompt and the image latent. For that, we use a lightweight, context-aware reward conditioning module. The $D$-dimensional vector $\gamma$ is first converted into a sequence of natural language tokens (e.g., ``first: win, second: tie''). 

\subsection{Mitigating Gradient Domination}
\label{subsec:reward_drop}
While our $L_{MC}$ objective~\Cref{eq:lmc} successfully disentangles reward axes, naively training with it can lead to gradient domination.
This occurs when dimensions that are easier to learn suppress the learning signals for harder dimensions, leading to unbalanced optimization. 


Under the reward decomposition at optimum (Eq.~\eqref{eq:reward_decomp}), analyzing the gradient of $L_{MC}$ reduces to an equivalent analysis of $L_M'$ (Eq.~\eqref{eq:lm_prime}), since the conditional policy $p_\theta(\mathbf{x}|c,\gamma)$ decomposes into the same per-dimension structure. We can write the gradient of the loss as follows:
%\vspace{-2mm}
\footnotesize
\begin{equation}
\begin{split}
    &\nabla_\theta L_M' = (\sigma (z)-1)\nabla_\theta z ,\\
    \nabla_\theta z = \sum_i\beta w_i &(\nabla_\theta \log p_\theta(\mathbf{x}^w|c,i) - \nabla_\theta \log p_\theta(\mathbf{x}^l|c,i)),
\end{split}
\end{equation}
\normalsize
where $z$ aggregates the per-dimension log-likelihood ratios. We can find two sources of the issue.
First, if any single dimension becomes highly confident, $\sigma(z) \rightarrow 1$, the global gradient goes to zero; therefore, the entire training converges to the local optima. Second, within $\nabla_\theta z$, if the model 
becomes highly discriminative for dimension $i$, which causes a large gradient norm for that dimension; it can dominate the sum and overwhelm gradients from other dimensions.

To address this, we introduce dimensional reward dropout. During training, we randomly drop individual reward dimensions by setting their condition $\gamma_i = 0$. By doing so, we can zero out the contribution of the dropped dimension to both the $\sigma(z)$ term and the summed gradient $\nabla_{\theta}z$. This simple technique prevents any single dimension from consistently dominating the training signal, ensuring balanced optimization across all axes.

\subsection{Test-time Reward Optimization}
\label{subsec:testtime}
A significant advantage of our conditional framework is that it enables dynamic, multi-axis reward optimization at inference time. Our training objective implicitly guides the model to represent two distinct distributions, including the distribution of preferred samples $p(\mathbf{x}|c,\gamma^w)$ and the distribution of non-preferred samples $p(\mathbf{x}|c,\gamma^l)$:
\small
\begin{equation}
    p(\mathbf{x}|c,\gamma^w) = p_{\text{ref}}(\mathbf{x}|c)\exp(r^w(\mathbf{x},c)/\beta)/Z(c).
    \label{eq:implicit}
\end{equation}
\normalsize

This structure is a natural fit for Classifier-Free Guidance (CFG). By computing the difference between the score functions for the ``win'' and ``lose'' conditions, we can derive the gradient of the implicit reward difference ($r^w - r^l$):
\small
\begin{equation}
    \nabla_\mathbf{x} \log\ p(\mathbf{x}|c,\gamma^w)-\nabla_\mathbf{x} \log\ p(\mathbf{x}|c,\gamma^l) = \nabla_\mathbf{x}( r^w- r^l)/\beta.
\end{equation}
\normalsize
The gradient can be incorporated into the standard CFG sampling as follows:
\small
\begin{equation}
\nabla_\mathbf{x} \log\ p(\mathbf{x}|\gamma^l) + \lambda_{cfg}(\nabla_\mathbf{x} \log\ p(\mathbf{x}|c,\gamma^w)-\nabla_\mathbf{x} \log\ p(\mathbf{x}|\gamma^l)).
\end{equation}
\normalsize
By doing so, we can steer the generation process away from the non-preferred ($\gamma^l$) and toward the preferred ($\gamma^w$). This enables fine-grained, dynamic control, allowing a user to specify a weighted combination of preference gradients at test time without requiring any external reward models.

\subsection{Context-aware Reward Conditioning}
\label{subsec:contextawaremodule}
We encode the preference outcome vector $\gamma$ as natural language tokens (e.g., ``win tie'', meaning win for the first (\eg, aesthetic) score and tie for the second (\eg, semantic alignment) via the text encoder to get an initial embedding $e_\gamma$. This embedding is then injected into the model.

First, the U-Net latent $z_t$ is updated using parallel cross-attention (CA) blocks with the text prompt $c_{\text{prompt}}$ and the final context-aware reward (CAR) embedding $c_{\text{reward}}$:
\begin{equation}
    z_t' = \text{CA}(z_t, c_{\text{prompt}}) + \lambda \cdot \text{CA}'(z_t, c_{\text{reward}}),
    \label{eq:ipadapter}
\end{equation}
where $z_t'$ is the updated latent, $\text{CA}'$ is a copy of the pretrained CA module~\cite{ye2023ipadapter}, and $\lambda$ is a weighting scalar, which we set to 1 in all our experiments.

For dimensions requiring both text and image context (e.g., semantic alignment), the embedding $c_{\text{reward}}$ is computed using a context-aware conditioning module. This module refines the initial $\gamma$ embedding $e_\gamma$ by attending to both the text prompt and the image latent sequentially:
\begin{equation}
    % \begin{split}
    h_{\text{SA}} = \text{SA}(e_\gamma, c_{\text{prompt}}), \ h_{\text{CA}} = \text{CA}''(h_{\text{SA}}, z_t), \
    c_{\text{reward}} = \text{MLP}(h_{\text{CA}}),
% \end{split}
\label{eq:car}
\end{equation}
where SA, $\text{CA}''$, and MLP are zero-initialized to preserve pretrained knowledge. This final $c_{\text{reward}}$ embedding is then fed into~\Cref{eq:ipadapter} as the input to $\text{CA}'$.

\noindent\textbf{Training Initialization} The modules introduced above ($\text{CA}'$ and the context-aware reward conditioning) are newly added parameters that are zero-initialized to preserve pretrained knowledge. As a result, the conditioning signal $\gamma$ has no effect at initialization.
Just as SFT before DPO in LLMs~\cite{rafailov2023dpo} helps the model
learn basic instruction-following before preference optimization,
we perform a supervised fine-tuning stage (MCSFT) that trains the conditioning
modules to reconstruct preferred samples $\mathbf{x}^w$ given $\gamma^w$
with a frozen U-Net, allowing the model to learn basic condition-following
before the MCDPO alignment begins.
% making direct MCDPO training unstable. To address this, we first perform a supervised fine-tuning stage (MCSFT) that trains the model to reconstruct preferred samples $\mathbf{x}^w$ conditioned on their corresponding preference vector $\gamma^w$ with frozen U-net. This stage allows the conditioning modules to learn a meaningful mapping from $\gamma$ to the reward-aware representation before the DPO alignment.
We emphasize that MCSFT serves solely as initialization, as shown in~\cref{tab:mainsdxl,tab:conflict}. MCSFT alone is insufficient and the subsequent MCDPO alignment stage is critical for final performance.

%%%%


\section{Experiments}
\label{sec:experiments}


\subsection{Experimental Setup}
\noindent\textbf{Training Dataset.}
% Pickapic-v2 dataset을 학습에 활용. MCSFT를 SD1.5에서 500스텝, SDXL에서 200step만 학습. lr은 1e-8 with batch scalining. 여기서 위의 context-aware reward module만 학습하고, diffusion model은 freeze. 그러고 MCDPO는 둘다 500step 학습, beta는 5000 사용, lr은 1e-9, 5e-9 with batch scalining. Batch size는 384, 64 각각 사용해서 학습함.
Following the previous works, we adopt Pick-a-Pic v2~\cite{kirstain2023pick}, containing 1M human-preference image pairs as the training dataset.
We augment each pair with four model-based reward dimensions: aesthetic quality (Aesthetic Predictor~\cite{laionaes}), semantic alignment (CLIP~\cite{radford2021learning}), overall quality (HPSv2~\cite{wu2023human}), and prompt alignment (PickScore~\cite{kirstain2023pick}).
For our method, the 5-dimensional preference outcome vector $\gamma$ is then constructed by encoding the win/lose/tie status for the original human label alongside these four proxy reward dimensions by discretizing into 100 bins (same bin = ties) after normalization on training dataset. We use 18\% of the data ($\sim$180K pairs) for StableDiffusion1.5 (SD1.5)~\cite{Rombach_2022_CVPR} and 3\% ($\sim$30K pairs) for SDXL~\cite{podell2023sdxl} compared to baselines.




% \begin{table}[t]
% \centering
% \small
% \begin{minipage}[t]{0.48\linewidth}
%     \centering
%     \caption{\textbf{Fair comparison across training regimes.} All models are trained on an identical 18\% data budget. MCDPO significantly outperforms all baselines, including filtered and conflict-only regimes, demonstrating its robust conflict resolution.}
%     \label{tab:conflict}
%     \vspace{-2mm}
%     \resizebox{0.95\linewidth}{!}{
% \begin{tabular}{l|cccccc|c} \hline
%                & Pick & Aes  & HPS  & CLIP & IR   & MPS  & Avg  \\ \hline
% (1) DPO            & 75.1 & 62.6 & 71.7 & 60.4 & 62.6 & 68.1 & 66.7 \\
% (2) DPO merged     & 73.4 & 63.5 & 70.0 & 56.1 & 62.0 & 67.9 & 63.8 \\
% (3) CDPO merged    & 63.4 & 84.8 & 71.7 & 32.3 & 61.1 & 65.0 & 63.1 \\
% (4) Filtered DPO   & 83.6 & 84.1 & 85.7 & 62.8 & 79.2 & 76.6 & 78.7 \\
% (5) MCSFT (full)   & 78.1 & 78.3 & 81.7 & 55.4 & 77.0 & 68.7 & 73.2 \\
% (6) MCDPO          & 86.2 & 91.8 & 93.4 & 57.6 & 82.9 & 76.7 & 81.1 \\
% (7) Conflict DPO   & 62.0 & 57.0 & 60.4 & 56.4 & 56.6 & 61.9 & 59.0 \\
% (8) Conflict MCDPO & 85.2 & 83.2 & 89.4 & 56.0 & 74.0 & 74.3 & 77.0 \\ \hline
% \end{tabular}
%     }
% \end{minipage}
% \hfill 
% \begin{minipage}[t]{0.48\linewidth}
%     \centering
%     \caption{Comparison of single-dimension DPO specialists trained without conditioning. We report win rates for each specialist, their parameter-averaged model (Merged), and our MCDPO for reference.}
%     \label{tab:single_dpo}
%     \vspace{-2mm}
%     \resizebox{0.95\linewidth}{!}{
% \begin{tabular}{l|cccccc|c}
% \hline
%           & Pick     & Aes     & HPS         & CLIP          & IR   & MPS           & Avg       \\ \hline
% Human     & {\ul 75.1}    & 62.6          & 71.7          & \textbf{60.4} & {\ul 62.6}    & {\ul 68.1}    & {\ul 66.7}    \\
% PickScore & 72.6          & 63.4          & {\ul 72.0}    & {\ul 59.2}    & 57.6          & 66.6          & 65.2          \\
% Aesthetic & 69.8          & {\ul 66.3}    & 66.4          & 56.4          & 59.5          & 66.0          & 64.1          \\
% HPSv2     & 69.8          & 63.9          & 70.1          & 54.5          & 59.5          & 65.9          & 64.0          \\
% CLIP      & 69.3          & 62.4          & 67.7          & 58.5          & 58.9          & 63.2          & 63.3          \\
% Merged    & 73.4          & 63.5          & 70.0          & 56.1          & 62.0          & 67.9          & 63.8          \\ \hline
% MCDPO     & \textbf{86.2} & \textbf{91.8} & \textbf{93.4} & 57.6          & \textbf{82.9} & \textbf{76.7} & \textbf{81.1} \\ \hline
% \end{tabular}
% \label{tab:singledim_dpo}
%     }
% \end{minipage}
% \end{table}


% \begin{table}[t]
% \centering
% \small
% \begin{minipage}[t]{0.49\linewidth}
%     \centering
%     \caption{Test-time reward axis interpolation.}
%     \label{tab:test_time_reward_axis}
%     \vspace{-2mm}
%     \resizebox{0.95\linewidth}{!}{
% \begin{tabular}{l|cccccc|c} \hline
%                    & Pick & Aes  & HPS  & CLIP & IR   & MPS  & Avg  \\\hline
% Human -- (1)       & 78.6 & 79.0 & 83.2 & 55.2 & 73.8 & 74.0 & 74.0 \\
% (1) + Pick -- (2)  & 83.1 & 81.5 & 88.4 & 57.2 & 76.9 & 72.0 & 76.5 \\
% (2) + Aes -- (3)   & 86.0 & 94.8 & 88.6 & 49.1 & 79.0 & 77.1 & 79.1 \\
% (3) + HPS -- (4)   & 89.9 & 94.7 & 91.3 & 52.0 & 80.3 & 79.0 & 81.2 \\
% (4) + CLIP (MCDPO) & 86.2 & 91.9 & 93.4 & 57.6 & 82.9 & 76.8 & 81.5 \\ \hline
% Aes-CLIP Control   & 88.0 & 90.6 & 91.2 & 59.6 & 81.0 & 78.4 & 81.5 \\ \hline
% \end{tabular}
%     }
% \end{minipage}
% \hfill 
% % --- 두 번째 테이블: Ablation CLIP Dropout
% \begin{minipage}[t]{0.49\linewidth}
%     \centering
%     \caption{Ablation on CLIP Dropout $p$}
%     \label{tab:ablation_clip_dropout}
%     \vspace{-2mm}
%     \resizebox{0.95\linewidth}{!}{
% \begin{tabular}{l|cccccc|c}
% \hline
%  & Pick & Aes & HPS & CLIP & IR & MPS & Avg \\ \hline
% $p=0.0$ & 85.5 & 91.7 & 93.2 & 57.3 & 83.3 & 76.2 & 81.2 \\
% $p=0.05$ & 86.4 & 91.1 & 92.9 & \textbf{57.8} & 82.7 & 76.1 & 81.2 \\
% $p=0.10$ & 86.2 & \textbf{91.9} & 92.8 & 57.2 & \textbf{83.7} & 76.5 & 81.4 \\
% $p=0.15$ (Ours) & 86.2 & \textbf{91.9} & \textbf{93.4} & 57.6 & 82.9 & 76.8 & \textbf{81.5} \\
% $p=0.20$ & 86.6 & 91.8 & \textbf{93.4} & 57.3 & 83.0 & 76.7 & \textbf{81.5} \\ \hline
% \end{tabular}
%     }
% \end{minipage}
% \end{table}
\tabmainSD
\tabmainSDXL

\noindent\textbf{Configuration.} Training proceeds in two phases: (1) MCSFT pre-training and (2) MCDPO alignment . The total computational time, including the prior MCSFT pretraining, was 16 and 32 A100 GPU hours for SD1.5 and SDXL, respectively. Other implementation details are provided in the Appendix.


\noindent\textbf{Evaluation.}
To evaluate MCDPO's effectiveness, we compare against existing baselines trained on the Pick-a-Pic v2 dataset: Diffusion-DPO~\cite{wallace2024ddpo}, Diffusion-KTO~\cite{lialigning}, MAPO~\cite{hong2024mapo}, and DSPO~\cite{zhu2025dspo}. Following standard convention, we test text-to-image generation on Pick-a-Pic v2 test set~\cite{kirstain2023pick}, PartiPrompts~\cite{yu2022scaling}, and HPDv2 test set~\cite{wu2023human}, measuring performance with PickScore, LAION Aesthetic Score, HPSv2, CLIP, ImageReward~\cite{xu2023imagereward}, and MPS~\cite{zhang2024learning}.

\subsection{Main Results}
% Table 1은 SD1.5에 대해서 Diffusion-DPO, Diffusion-KTO, DSPO and MCDPO의 win rate을 보여준다. MCDPO는 모든 testset에서 압도적인 성능을 보인다. Pickscore, HPS, 둘다 꽤 많은 점수가 오르고, 특히 aesthetic score의 경우 기존 대비 매우 많이 성능의 gain이 존재한다. 그리고 Reward Dimension으로 직접적으로 활용되지 않은 ImageReward에서도 consistently 성능의 gain이 존재한다. SDXL에서도 MCDPO는 significantly 성능의 gain을 보인다. HPS PickScore에서는 모든 경우 baseline들 보다 좋고, 평균점수도 굉장히 높다.
As shown in \Cref{tab:mainsd}, our method, MCDPO, demonstrates dominant performance on the SD1.5 benchmark, significantly outperforming all baselines (Diffusion-DPO, Diffusion-KTO, and DSPO) across every test set. We observe substantial gains in both PickScore and HPSv2. The most notable improvement is in the
\begin{wraptable}{r}{0.5\textwidth}
  % \vspace{-\intextsep} % 위쪽 여백 강제 제거 (그림과 동일한 팁 적용)
  \centering
  \vspace{-4mm}  
  \caption{\textbf{Fair comparison across training regimes.} All models are trained on an identical 18\% data budget. MCDPO significantly outperforms all baselines, including filtered and conflict-only regimes, demonstrating its robust conflict resolution.}
    \label{tab:conflict}
    \resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cccccc|c} \hline
               & Pick & Aes  & HPS  & CLIP & IR   & MPS  & Avg  \\ \hline
(1) DPO            & 75.1 & 62.6 & 71.7 & {\ul 60.4} & 62.6 & 68.1 & 66.7 \\
(2) DPO merged     & 73.4 & 63.5 & 70.0 & 56.1 & 62.0 & 67.9 & 63.8 \\
(3) CDPO merged    & 63.4 & {\ul 84.8} & 71.7 & 32.3 & 61.1 & 65.0 & 63.1 \\
(4) Filtered DPO   & 83.6 & 84.1 & 85.7 & \textbf{62.8} & {\ul 79.2} & {\ul 76.6} & {\ul 78.7} \\
(5) MCSFT (full)   & 78.1 & 78.3 & 81.7 & 55.4 & 77.0 & 68.7 & 73.2 \\
(6) MCDPO          & \textbf{86.2} & \textbf{91.8} & \textbf{93.4} & 57.6 & \textbf{82.9} & \textbf{76.7} & \textbf{81.1} \\
(7) Conflict DPO   & 62.0 & 57.0 & 60.4 & 56.4 & 56.6 & 61.9 & 59.0 \\
(8) Conflict MCDPO & {\ul 85.2} & 83.2 & {\ul 89.4} & 56.0 & 74.0 & 74.3 & 77.0 \\ \hline
\end{tabular}}
  \vspace{-14pt}
\end{wraptable}
aesthetic score, which shows a massive performance gain over existing methods. Furthermore, MCDPO achieves consistent gains on ImageReward and MPS, metrics not used as a direct reward dimension, indicating strong generalization capabilities.
This significant performance advantage is maintained on SDXL, as detailed in \Cref{tab:mainsdxl}. MCDPO again outperforms all baselines on PickScore, HPSv2, and MPS, achieving the highest average score by a large margin.

% While MCDPO achieves substantial improvements across human-preference metrics, CLIP scores show comparable that warrant explanation. Importantly, \Cref{tab:singledim_inf} demonstrates that MCDPO successfully learns CLIP optimization.
% When applying test-time guidance targeting CLIP specifically, our model achieves 59.0\%, notably higher than baseline DPO (57.8\%).
% This proves the model has learned a disentangled CLIP representation.
% However, when optimizing all dimensions simultaneously, CLIP score moderates to 57.6\%. This reflects the fundamental nature of multi-objective optimization. Achieving peak performance across all metrics simultaneously requires balanced compromise.
% The slight moderation in
% CLIP (while remaining competitive with baselines) enables dramatic improvements in aesthetics (91.8\%), HPSv2 (93.4\%), ImageReward (82.9\%), and MPS (76.7\%). Critically, our conditional framework allows users to dynamically adjust this trade-off at inference, boosting CLIP to 59.0\% when semantic alignment is prioritized, or maximizing aesthetics when preferred. Furthermore, our framework enables temporal reward scheduling. By setting the aesthetic condition to `tie' for the initial 25 steps and `win' for the remaining 25, we can further boost the CLIP score, explicitly trading a slight decrease in aesthetic quality for improved semantic alignment in~\Cref{tab:singledim_inf}.

While MCDPO achieves substantial improvements across human-preference metrics, CLIP scores are slightly lower than standard DPO. This reflects a natural multi-objective trade-off, where the moderate CLIP enables dramatic gains in aesthetics (91.9\%), HPSv2 (93.4\%), ImageReward (82.9\%), and MPS (76.7\%). Importantly, \Cref{tab:singledim_inf} confirms that MCDPO has learned a disentangled CLIP representation that can be amplified at test-time. In~\Cref{tab:singledim_inf}, targeting CLIP alone yields 59.0\%, and Aes-CLIP temporal scheduling, which assigns aesthetic `tie' for the first 25 steps and `win' for the remaining 25, further recovers the gap to 59.6\% while preserving the highest overall average (81.5\%).


% However, we observe that the CLIP score is either comparable or slightly lower than the baselines. We hypothesize this stems from three potential factors; (1) Aesthetic vs. CLIP Trade-off: A well-documented trade-off between aesthetic quality and CLIP score has been reported in prior research.[\textbf{cite}] Heavily optimizing for aesthetics, as our model does, often leads to stylistic changes in the generated images, which can negatively impact the CLIP score's measure of text-image alignment. This effect is clearly visible in the MAPO baseline, which achieves a high aesthetic score at the cost of a severe drop in its CLIP score. (2) Noisy Reward Guidance: The reliability of the CLIP score as a robust reward signal has been questioned in several studies.~\cite{} It is possible that when used as a direct reward, its inherent noise and biases may not be a clear optimization signal. (3) Weakened Text Conditioning: The introduction of our additional reward vector as a condition might slightly dilute the model's focus on the primary text prompt conditioning. We provide further analysis of this conditioning mechanism in \Cref{subsec:contextawaremodule}.

% 4.1에서 언급했다시피, 다른 baseline들 대비 ours의 경우 SD1.5는 18\%, SDXL의 경우 3\%의 data만을 활용하여 학습했음에도 불구하고 굉장히 높은 성능을 보인다. 이는 disentangled bradley-terry를 modeling할 수 있는 mcdpo의 특성에서 기인하는 장점이라 생각한다. Fig.x는 이를 확인하기 위해 우리는 모든 reward dimension이 align되어있는 data만을 Pickapic-v2에서 filtering하여 DPO를 통해 학습한 모델과 성능을 비교한다. 이때 filtering된 데이터는 전체 데이터의 18\% 정도이며 dpo와 mcdpo는 무작위로 동일한 18\% 데이터를 샘플링하여 학습하였다. 보다시피 reward conflict를 제거한 DPO-filtered는 기존 DPO대비 매우 높은 성능의 gain을 보였음에도 불구하고, MCDPO가 더 높은 성능을 보인다. 이는 MCDPO가 noisy한 data에서도 매우 effective한 learning signal을 흘려줄 수 있을지를 보여준다.


To ensure a fair comparison across various training regimes, we evaluate our method using an identical 18\% subset of the Pick-a-Pic v2 dataset. \Cref{tab:conflict} compares eight distinct configurations to demonstrate how effectively MCDPO resolves reward conflicts. (1) Standard DPO on randomly sampled pairs, (2)
merged checkpoints of DPO models trained independently on each reward axis — same supervision, (3) merged checkpoints of Conditional DPO (CDPO) models independently trained on each axis — same supervision and parameters (4) DPO-Filtered on conflict-free pairs only, (5) full MCSFT training (unfreezing the U-Net after the initial MCSFT phase) — same supervision and parameters (6) our proposed MCDPO on randomly sampled pairs, (7) DPO trained strictly on conflict-only pairs, and (8) MCDPO trained strictly on conflict-only pairs.

\figQualSD
\figQualSDXL

Notably, MCDPO surpasses DPO-Filtered, which explicitly avoids conflicting signals by discarding 82\% of training data, demonstrating that MCDPO successfully transforms conflict pairs from obstacles into highly effective training signals. Furthermore, we observe that full MCSFT training alone actually degrades performance, confirming that the MCDPO alignment objective is indispensable for stable optimization.
To explicitly demonstrate that our model fundamentally resolves reward conflicts, we compare the models trained exclusively on conflicting pairs ((7) and (8)).
When restricted to conflict-only data, standard DPO suffers a substantial relative performance degradation of 11.5\% compared to its randomly sampled baseline. In contrast, MCDPO experiences a minor drop of only 5.1\%. It underscores MCDPO's superior efficiency in extracting disentangled learning signals even from highly contradictory data.

Remarkably, the conflict-trained MCDPO maintains high performance even when conditioned on ``all-win'' across every dimension, a scenario never encountered during training. We provide further analysis in~\Cref{fig:reward_traj} and agreement ratio over reward dimensions in appendix.
% Remarkably, the conflict-trained MCDPO model maintains high performance during inference even when conditioned on an ``all-win'' state across every dimension an optimal scenario it never once encountered during training. To further support these findings, we provide implicit reward measurements for the conflict samples in~\Cref{fig:reward_traj} and detail the agreement ratios of the generated samples in the appendix.

Furthermore, we visualize the qualitative result of MCDPO against baseline methods on both SD1.5 and SDXL, in~\Cref{fig:qual_sd15} and~\Cref{fig:qual_sdxl}, respectively.
Across both models, our method demonstrates a clear superiority in generating images that are more aesthetically pleasing and detailed.



% \tabAblationPick
\subsection{Analysis}

% \noindent\textbf{Multi-dimensional Learning.} \Cref{tab:singledim_dpo,tab:singledim} validates the effectiveness of our
% multi-dimensional learning approach by comparing MCDPO, trained on all reward dimensions simultaneously, against specialist models trained on a single reward dimension. To evaluate the independent modeling approach defined in Eq.~\eqref{eq:lm}, \Cref{tab:singledim_dpo} reports the performance of models trained independently on each reward axis following the standard DPO objective with identical hyperparameters. Similarly, \Cref{tab:singledim} presents models trained for each specific reward using the Conditional DPO paradigm, utilizing the exact same parameters and hyperparameters as our full MCDPO.

\noindent\textbf{Multi-dimensional Learning.} \Cref{tab:singledim_dpo,tab:singledim} compare MCDPO against specialist models trained on a single reward axis,
using both the standard DPO objective (\Cref{tab:singledim_dpo}) and our Conditional DPO paradigm with identical architecture and hyperparameters (\Cref{tab:singledim}).


Remarkably, the MCDPO model not only achieves the highest average score but also outperforms every individual specialist model on its own specialized metric, with the sole exception of the CLIP score in~\Cref{tab:singledim_dpo}. For example, the MCDPO model (Aesthetic win-rate 91.8\%) significantly surpasses the model trained exclusively on `Aesthetic' rewards (Aesthetic win-rate 88.1\%) in~\Cref{tab:singledim}.

We conjecture that MCDPO mitigates potential training reward overfitting by leveraging cross-dimensional references to learn robust features rather than train-specific shortcuts. For example, one dimension may exploit spurious cues that improve training reward but harm semantics. The CLIP dimension can provide a semantic reference that helps mitigate this.

% This finding strongly substantiates our core hypothesis. It suggests that training DPO on even a single dimension still fails to achieve optimal performance due to implicit reward conflicts with other unstated dimensions. The model struggles because it cannot resolve these conflicts that it is not conditioned to understand.
% In contrast, MCDPO resolves this issue by explicitly conditioning on and disentangling all potential conflict axes. This allows the model to properly optimize each dimension individually, which leads to state-of-the-art performance across all metrics.


% \tabSingleDim
% \tabSingleDimAblationPick

\begin{table}[t]
\centering
% \small
% --- 두 번째 테이블: Ablation Pick
\begin{minipage}[t]{0.49\linewidth}
    \centering
    \caption{\textbf{Standard DPO specialists.}}
    \label{tab:single_dpo}
    \vspace{-2mm}
    \resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|cccccc|c}
\hline
          & Pick     & Aes     & HPS         & CLIP          & IR   & MPS           & Avg       \\ \hline
Human     & {\ul 75.1}    & 62.6          & 71.7          & \textbf{60.4} & {\ul 62.6}    & {\ul 68.1}    & {\ul 66.7}    \\
Pick & 72.6          & 63.4          & {\ul 72.0}    & {\ul 59.2}    & 57.6          & 66.6          & 65.2          \\
Aes & 69.8          & {\ul 66.3}    & 66.4          & 56.4          & 59.5          & 66.0          & 64.1          \\
HPS     & 69.8          & 63.9          & 70.1          & 54.5          & 59.5          & 65.9          & 64.0          \\
CLIP      & 69.3          & 62.4          & 67.7          & 58.5          & 58.9          & 63.2          & 63.3          \\
Merged    & 73.4          & 63.5          & 70.0          & 56.1          & 62.0          & 67.9          & 63.8          \\ \hline
MCDPO     & \textbf{86.2} & \textbf{91.8} & \textbf{93.4} & 57.6          & \textbf{82.9} & \textbf{76.7} & \textbf{81.1} \\ \hline
\end{tabular}
\label{tab:singledim_dpo}
    }
\end{minipage}
\hfill 
\begin{minipage}[t]{0.49\linewidth}
    \centering
    \caption{\textbf{Cond. DPO specialists.}}
    \label{tab:singledim}
    \vspace{-3mm}
    \resizebox{0.99\linewidth}{!}{
        \begin{tabular}{l|cccccc|c} \hline
         & Pick & Aes  & HPS  & CLIP & IR & MPS   & Avg  \\ \hline
        Human  & 79.0 & 79.8 & 86.5 & 46.8 & 75.9 & 73.2 & 73.5 \\
        Pick   & {\ul 80.7} & 82.8 & {\ul 88.5} & 49.0 & 76.8 & {\ul 74.7} & {\ul 75.4} \\
        Aes    & 79.6 & {\ul 88.1} & 87.2 & 49.1 & 76.2 & 72.5 & {\ul 75.4} \\
        HPS    & 77.8 & 81.8 & 88.0 & {\ul 50.2} & {\ul 77.6} & 73.3 & 74.7 \\
        CLIP   & 75.3 & 79.3 & 84.5 & 49.3 & 76.0 & 70.9 & 72.5 \\
        Merged   & 63.4 & 84.8 & 71.7 & 32.3 & 61.1 & 65.0 & 63.1 \\ \hline
        MCDPO    & \textbf{86.2} & \textbf{91.8} & \textbf{93.4} & \textbf{57.6} & \textbf{82.9} & \textbf{76.7} & \textbf{81.1} \\ \hline
        \end{tabular}
    }
\end{minipage}
\vspace{-5mm}
\end{table}


\noindent\textbf{Multi-dimensional Inference.}
As demonstrated in~\Cref{tab:singledim_inf}, our single model, trained to disentangle reward axes, can perform dynamic preference-enhancing sampling at test-time as described in~\Cref{subsec:testtime}. When steering the sampling to amplify only a specific or multiple dimensions, we observe distinct and controlled behaviors. Critically, when enhancing CLIP, the model achieves 59.0\%, recovering from the all-dimension default (57.6\%) and demonstrating that MCDPO has learned a disentangled CLIP representation that can be amplified when desired.
% \begin{wraptable}{l}{0.5\textwidth}
%   % \vspace{-\intextsep} % 위쪽 여백 강제 제거 (그림과 동일한 팁 적용)
%   \centering
%   \vspace{-7mm}  
%   \caption{Test-time reward optimization by guiding the MCDPO model towards specific target dimensions.}
%     \label{tab:singledim_inf}
%     % \vspace{-2mm}
%     \resizebox{0.99\linewidth}{!}{
%         \begin{tabular}{l|cccccc|c} \hline
%          & Pick          & Aes           & HPS           & CLIP          & IR       & MPS     & Avg           \\ \hline
%         Human & {\ul 78.6}    & 79.0          & 83.3          & 55.2          & 73.7      & 67.7    & 72.9          \\
%         Pick  & 78.1          & 79.0          & 85.1          & {\ul 57.6}    & {\ul 78.4} & 69.9   & 74.7          \\
%         Aes   & 77.3          & \textbf{95.8} & 79.1          & 49.3          & 73.1     & 68.8     & 73.8          \\
%         HPS   & 77.0          & 79.5          & {\ul 85.6}    & \textbf{59.0} & 77.8     & {\ul 71.1}     & {\ul 74.9}    \\
%         CLIP  & 76.4          & 76.5          & 85.1          & \textbf{59.0} & 75.0    & 67.8      & 73.3          \\ \hline
%         Aes-CLIP Cont.   & 88.0 & 90.6 & 91.2 & 59.6 & 81.0 & 78.4 & 81.5 \\
%         ALL   & \textbf{86.2} & {\ul 91.8}    & \textbf{93.4} & {\ul 57.6}    & \textbf{82.9} & \textbf{76.7} & \textbf{81.1} \\ \hline
%         \end{tabular}
%     }
%   \vspace{-14pt}
% \end{wraptable}
% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-3mm}
% \centering
% \includegraphics[width=0.99\linewidth]{figure/combined_acc_trajectory_horizontal.png}
% \vspace{-6mm}
% \caption{Implicit reward accuracy on Human-Aesthetic conflict-only pairs.}
% \label{fig:reward_traj}
% \vspace{-14pt}
% \end{wrapfigure}


\begin{figure}[t]
    \centering
    
    % --- 왼쪽: 표 배치 ---
    \begin{minipage}[c]{0.48\textwidth}
        \centering
        % \captionof를 사용하면 figure 환경 안에서도 Table 캡션을 달 수 있습니다.
        \captionof{table}{Test-time reward optimization by guiding the MCDPO model towards specific target dimensions.}
        \label{tab:singledim_inf}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{l|cccccc|c} \hline
                & Pick    & Aes           & HPS           & CLIP          & IR       & MPS     & Avg           \\ \hline
                Human & {\ul 78.6} & 79.0          & 83.3          & 55.2          & 73.7      & 67.7    & 72.9          \\
                Pick  & 78.1       & 79.0          & 85.1          & {\ul 57.6}    & {\ul 78.4} & 69.9   & 74.7          \\
                Aes   & 77.3       & \textbf{95.8} & 79.1          & 49.3          & 73.1     & 68.8     & 73.8          \\
                HPS   & 77.0       & 79.5          & {\ul 85.6}    & \textbf{59.0} & 77.8     & {\ul 71.1}     & {\ul 74.9}    \\
                CLIP  & 76.4       & 76.5          & 85.1          & \textbf{59.0} & 75.0    & 67.8      & 73.3          \\ \hline
                Aes-CLIP Cont.   & 88.0 & 90.6 & 91.2 & 59.6 & 81.0 & 78.4 & 81.5 \\
                ALL   & \textbf{86.2} & {\ul 91.8}    & \textbf{93.4} & {\ul 57.6}    & \textbf{82.9} & \textbf{76.7} & \textbf{81.1} \\ \hline
            \end{tabular}
        }
    \end{minipage}% <--- 이 부분에 빈 줄이 없어야 합니다!
    \hfill % 두 minipage 사이의 간격을 자동으로 띄워줍니다.
    % --- 오른쪽: 그림 배치 ---
    \begin{minipage}[c]{0.48\textwidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{figure/combined_acc_trajectory_horizontal.png}
        \captionof{figure}{Implicit reward accuracy on Human-Aesthetic conflict-only pairs.}
        \label{fig:reward_traj}
    \end{minipage}
    \vspace{-5mm}
\end{figure}

This demonstrates that MCDPO has successfully learned a disentangled representation of CLIP rewards and can boost this dimension when desired.
Similarly, enhancing Aes (Aesthetic) generates samples with exceptionally high aesthetic scores (95.8\%), validating dimension-specific control.


Notably, when enhancing PickScore and HPSv2, their corresponding scores increase as expected. However, we also observe a concurrent rise in CLIP, ImageReward, and MPS scores.
We attribute this to the nature of PickScore and HPSv2 as holistic metrics that evaluate overall image quality, which naturally correlates with other reward axes.



While coarse axis-level optimization is detailed in the supplementary material, we highlight MCDPO's capability for fine-grained temporal control.
To mitigate the natural trade-off between aesthetics and semantics, we leverage the step-wise frequency properties of diffusion models. Semantic structures primarily form during early low-frequency steps, whereas aesthetic details emerge in later high-frequency steps. By assigning an aesthetic tie for the first 25 steps and a win condition for the remaining 25 steps, our Aes-CLIP Control (\Cref{tab:singledim_inf}) significantly boosts the CLIP score while maintaining the average win rate. We further provide an incremental analysis in Appendix, where adding each reward axis as ``win'' progressively improves the corresponding metric, confirming that each dimension contributes independently to the final performance.

% \Cref{tab:test_time_reward_axis}에서는 reward axis가 좋아지는 방향으로 하나씩 추가할때마다, 해당 dimension과 average winrate가 증가하는 경향성을 보인다. 다만 (3)에서 aesthetic이 추가될때 CLIP score에서 significant한 drop이 발생하는 것으로 미루어 보았을때, aesthetic 과 semantic에서 trade off가 있음을 추측할 수 있다. 이러한 trade off를 reward axis 단위에서 corase 하게만 조절할 수 있을 뿐만이 아니라, 더 fine하게도 이를 조절할 수 있다. Aes-CLIP Control의 경우 semantic을 형성하는데 더 민감한 low frequency denoising step (첫 25step)에서 aesthetic만 tie로 설정해 optimize하지 않고, 그 뒤에 high frequency denoising step (후반 25step)에서 aesthetic score까지 포함해서 optimize하여 동일한 avg win rate이지만 significantly clip win rate을 높일 수 있음을 보였다.


\noindent\textbf{Implicit Reward Modeling}
~\Cref{tab:implicit} demonstrates that MCDPO accurately models implicit reward functions for each dimension. MCDPO achieves comparable accuracy to specialist models trained on individual dimensions, while being significantly more computationally efficient by learning all dimensions within a single network.
Furthermore, our conditional DPO framework simultaneously models both $r^w$ (preferred) and $r^l$ (non-preferred) implicit reward models as described in~\Cref{eq:implicit}. Leveraging both models together yields performance gains over using either model alone. For example, in the Aesthetic dimension, while the win-only model achieves 50.8\% and the lose-only model achieves 53.3\%, combining both models substantially improves accuracy to 66.2\%. Similarly, for Human and PickScore dimensions, despite the lose models showing relatively lower accuracies (42.2\% and 41.0\% respectively), combining them with the win models consistently yields performance improvements.

\noindent\textbf{Reward Conflicts}
To demonstrate that MCDPO actively resolves reward conflicts beyond mere dimensional disentanglement, we plot the implicit rewards during training, on a filtered subset where Human and Aesthetic preferences conflict \Cref{fig:reward_traj}.
While standard DPO and Conflict DPO suffer active aesthetic feature degradation dropping to 35\% and 30\% respectively, MCDPO successfully rectifies the gradient direction via its axis-wise guidance $\gamma$. This isolates the aesthetic dimension from the global penalty and enables convergence towards the ideal disentangled distribution $p_{BT}^\perp$.

\begin{table}[!t]
\centering
% \small
% --- 두 번째 테이블: Ablation Pick
\begin{minipage}[t]{0.49\linewidth}
    \centering
    \caption{Implicit reward accuracy comparison between MCDPO and specialist.}
    \label{tab:implicit}
    \vspace{-2mm}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|ccccc} \hline
               & Human & Pick & Aes  & HPS  & CLIP \\ \hline
    % Diff. DPO  & 60.2  & \multicolumn{4}{c}{-}     \\
    Specialists & 57.8  & 61.0 & 67.1 & 58.2 & 59.9 \\
    MCDPO      & 58.7  & 61.7 & 66.2 & 55.0 & 59.4 \\ \hline
    MCDPO win  & 58.5  & 58.7 & 50.8 & 52.9 & 59.4 \\
    MCDPO lose & 42.2  & 41.0 & 53.3 & 46.8 & 56.8 \\ \hline
    \end{tabular}
    }
\end{minipage}
\hfill 
\begin{minipage}[t]{0.49\linewidth}
    \centering
    \caption{Ablation study of MCDPO components on PickV2.}
    \label{tab:ablation}
    \vspace{-2mm}
    \resizebox{0.95\linewidth}{!}{
        \begin{tabular}{l|cccccc|c} \hline
                        & Pick & Aes & HPS  & CLIP & IR  & MPS & Avg \\ \hline
        MCDPO           & {\ul 86.2}  & 91.8 & \textbf{93.4} & \textbf{57.6} & \textbf{83.0} & {\ul 76.7} & \textbf{81.1} \\ \hline
        reward dropout 0.1   & 85.8  & {\ul 93.5} & {\ul 92.4} & {\ul 55.6} & {\ul 82.4} & 74.8 & {\ul 80.7} \\
        reward dropout 0.0   & \textbf{87.3}  & \textbf{96.0} & 92.1 & 49.2 & 79.2 & \textbf{77.1} & 80.1 \\
        w/o MCSFT         & 53.8  & 79.2 & 55.1 & 48.8 & 55.7 & 70.7 & 60.5 \\
        w/o CAR module & 80.1  & 90.0 & 80.7 & 45.7 & 69.8 & 54.4 & 70.1 \\ \hline
        \end{tabular}
    }
\end{minipage}
\vspace{-4mm}
\end{table}

% Specialist conditional model들과 mcdpo가 각 reward dimension에서 implicit reward accuracy를 잘 측정할 수 있는지를 ~\Cref{tab:implicit}에서 보인다. 각각의 dimension에 대해서 학습한 specialist model들과 MCDPO는 각 dimension에 대해서 comparable한 accuracy를 보이며 이는 significantly computatation efficienct하게 각 dimension에 대해 학습이 잘 이뤄졌다는 것을 보인다. 또한 우리가 제안한 conditional DPO framework는~\Cref{eq:implicit} 처럼 $r^w$와 $r^l$에 해당하는 implicit reward 모델을 동시에 모델링하는데, 두 모델을 동시에 활용하여 implicit reward를 모델링 하였을때 하나의 모델만 활용한 것보다 성능의 gain이 존재함을 볼 수 있다. 특히 Aes의 경우 win model이 50.8, lose model이 53.3으로 다소 낮은 성능을 보이지만, 이를 같이 활용하는 경우 66.2로 굉장히 높은 성능을 보인다. 그리고 Human과 Pick에서 lose모델은 각각 42.2, 41.0으로 다소 낮은 결과를 보이는데, 그럼에도 불구하고, win model과 합쳐졌을 때에는 항상 성능의 gain이 존재한다.


\noindent\textbf{Component Ablation Study.} We conduct an ablation study to validate the contribution of MCDPO's core components: dimensional reward dropout, the context-aware reward module, and the MCSFT pre-training stage in~\Cref{tab:ablation}

First, removing the dimensional reward dropout leads to a seemingly 
dominant aesthetic score (95.8\%) but causes a catastrophic collapse in the CLIP score (49.3\%). We believe this is a clear case of the gradient domination problem discussed in \Cref{subsec:reward_drop}. The easier aesthetic dimension appears to saturate the learning signal, preventing the harder CLIP dimension from being optimized. Our reward dropout technique effectively mitigates this issue, ensuring balanced optimization and contributing significantly to the superior overall performance. Applying a reward dropout of just 0.1 significantly mitigates this domination.

Removing MCSFT pre-training causes a drastic performance decline, showing non-initialized conditioning is disruptive. However, MCSFT alone is insufficient. On SDXL, MCSFT performs poorly (Avg 57.13), while the full MCDPO model achieves 72.01 (\Cref{tab:mainsdxl}), proving the MCDPO alignment stage itself is critical.

Finally, ablating the Context-Aware Reward conditioning module Eq.~\eqref{eq:car} causes a severe performance drop in all metrics except for aesthetics. These affected metrics (PickScore, HPS, CLIP, IR) measure alignment between the image and the text prompt. This result confirms our hypothesis: to condition on rewards like semantic alignment effectively, the model must be aware of both the image and the text context, validating the design of our module.

% \Cref{tab:ablation_clip_dropout}은 global dropout rate은 0.2로 설정하고, clip의 dropout만을 조절한 결과이다. CLIP이 상대적으로 weak dimension이라 학습 기회를 많이 부여하기 위해서 drop rate을 낮춰 보았을때 clip dimension에 다소간의 gain이 있었지만 significant하지는 않았다.

% \tabSingleDimInf
% \tabImplicitReward

% \tabTestTimeRewardImplicitReward

\section{Conclusion}
\label{sec:conclusion}

% \noindent\textbf{Conclusion.} We introduced Multi Reward Conditional DPO (MCDPO), a framework that fundamentally resolves the reward conflict inherent in the standard Bradley-Terry formulation. By explicitly conditioning on preference outcome vectors, our approach transforms conflicting data pairs into robust training signals for disentangled alignment. Empirical results confirm that MCDPO achieves state-of-the-art performance and superior sample efficiency. Ultimately, this conditional framework offers a scalable and unified solution for precise and multi-dimensional control in generative model alignment.

% \noindent\textbf{Limitations.} While MCDPO effectively disentangles reward axes, the method relies on the availability of reliable proxy reward models to construct the preference outcome vector during training. The quality of the final alignment is therefore upper-bounded by the accuracy of these proxy judges. Additionally, unlike standard DPO, which utilizes binary human labels directly, our approach introduces a preprocessing overhead to generate multi-dimensional reward scores for the training data. 

We introduced Multi Reward Conditional DPO (MCDPO), a framework that resolves the reward conflict in the Bradley-Terry formulation by conditioning on preference outcome vectors, transforming conflicting pairs into robust training signals for disentangled alignment. MCDPO achieves state-of-the-art performance with superior sample efficiency, and enables dynamic multi-dimensional control at inference without additional training or external reward models. One limitation is the reliance on proxy reward models to construct the preference outcome vector, which upper-bounds alignment quality by their accuracy, and introduces preprocessing overhead compared to standard DPO's binary labels.


\bibliographystyle{splncs04}
\bibliography{main}
\end{document}
